Estimating On-road Transportation Carbon Emissions from Open Data of Road Network and Origin-destination Flow Data

Accounting for over 20% of the total carbon emissions, the precise estimation of on-road transportation carbon emissions is crucial for carbon emission monitoring and efficient mitigation policy formulation. However, existing estimation methods typically depend on hard-to-collect individual statistics of vehicle miles traveled to calculate emissions, thereby suffering from high data collection difficulty. To relieve this issue by utilizing the strong pattern recognition of artificial intelligence, we incorporate two sources of open data representative of the transportation demand and capacity factors, the origin-destination (OD) flow data and the road network data, to build a hierarchical heterogeneous graph learning method for on-road carbon emission estimation (HENCE). Specifically, a hierarchical graph consisting of the road network level, community level, and region level is constructed to model the multi-scale road network-based connectivity and travel connection between spatial areas. Heterogeneous graphs consisting of OD links and spatial links are further built at both the community level and region level to capture the intrinsic interactions between travel demand and road network accessibility. Extensive experiments on two large-scale real-world datasets demonstrate HENCE's effectiveness and superiority with R-squared exceeding 0.75 and outperforming baselines by 9.60% on average, validating its success in pioneering the use of artificial intelligence to empower carbon emission management and sustainability development. The implementation codes are available at this link: https://github.com/tsinghua-fib-lab/HENCE.

==> 3.preliminaries.tex <==
\section{Problem Formulation}
The goal of this work is to predict regional on-road carbon emissions with road network and origin-destination (OD) flow data, which represent the transportation demand and capacity factors respectively. Specifically, for a region set $\mathcal{A}$, we are given the road network $\bm{G_i}=(\bm{V_i}, \bm{E_i})$ for region $i\in \mathcal{A}$ where $\bm{V_i}$ and $\bm{E_i}$ refers to the road intersections and segments inside the region. We are also provided with OD flow statistics of the regions over a time span. Denoting all OD flows related to region $i$ as $\bm{O_i}$, the task is to build a prediction model to predict the region's transportation on-road carbon emissions $Y_i\in \mathbb{R}$ over this time period. The task can be formulated below,

\begin{equation}
    Y_i = f_{\bm{H}}\big(\bm{G_i}, \bm{O_i}\big).
\end{equation}


